Compositional Value Iteration with Pareto Caching

The de-facto standard approach in MDP verification is based on value iteration (VI). We propose compositional VI, a framework for model checking compositional MDPs, that addresses efficiency while maintaining soundness. Concretely, compositional MDPs naturally arise from the combination of individual components, and their structure can be expressed using, e.g., string diagrams. Towards efficiency, we observe that compositional VI repeatedly verifies individual components. We propose a technique called Pareto caching that allows to reuse verification results, even for previously unseen queries. Towards soundness, we present two stopping criteria: one generalizes the optimistic value iteration paradigm and the other uses Pareto caches in conjunction with recent baseline algorithms. Our experimental evaluations shows the promise of the novel algorithm and its variations, and identifies challenges for future work.

==> plots-backup/macros.tex <==

%% PLOTS
\newcommand{\scatterplotsize}[0]{1.2\textwidth}
\newcommand{\marksize}{1.8}

% Arguments:
% 1) csv file
% 2) csv column for data on x-axis
% 3) x-axis label
% 4) csv column for data on y-axis
% 5) y-axis label
\newcommand{\scatterplot}[5]{%
	\begin{tikzpicture}
	\begin{axis}[
	width=\scatterplotsize,
	height=\scatterplotsize,
	axis equal image,
	xmin=1,
	ymin=1,
	ymax=9000,
	xmax=9000,
	xmode=log,
	ymode=log,
	axis x line=bottom,
	axis y line=left,
	xtick={1,9,90,900},
	xticklabels={1,9,90,900},
	extra x ticks = {2700},
	extra x tick labels = {OoR},
	extra x tick style = {grid = major},
	ytick={1,9,90,900},
	yticklabels={1,9,90,900},
	extra y ticks = {2700},
	extra y tick labels = {OoR},
	extra y tick style = {grid = major},
	xlabel={\scriptsize #3},
	xlabel style={yshift=0cm},
	ylabel={\scriptsize #5},
	ylabel style={yshift=-0.4cm},
	yticklabel style={font=\tiny},
	xticklabel style={rotate=290,anchor=west,font=\tiny},
 legend pos=outer north east,
 %legend cell align=left,
	]

	\addplot[ % BiroomsBig
	scatter,
	only marks,
	mark=asterisk,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_0.csv};

	\addplot[ % BiroomsSmall
	scatter,
	only marks,
	mark=triangle,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_1.csv};

	\addplot[ % ChainsBig
	scatter,
	only marks,
	mark=square,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_2.csv};

	\addplot[ % ChainsDice3
	scatter,
	only marks,
	mark=diamond,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_3.csv};

	\addplot[ % ChainsDice4
	scatter,
	only marks,
	mark=-,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_4.csv};

	\addplot[ % ChainsDice5
	scatter,
	only marks,
	mark=|,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_5.csv};

	\addplot[ % ChainsDiceLoop3
	scatter,
	only marks,
	mark=Mercedes star,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_6.csv};

	\addplot[ % ChainsDiceLoop4
	scatter,
	only marks,
	mark=Mercedes star flipped,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_7.csv};

	\addplot[ % ChainsDiceLoop5
	scatter,
	only marks,
	mark=heart,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_8.csv};

	\addplot[ % ChainsSmall
	scatter,
	only marks,
	mark=pentagon,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_9.csv};

	\addplot[ % RoomsBig
	scatter,
	only marks,
	mark=oplus,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_10.csv};

	\addplot[ % RoomsDice
	scatter,
	only marks,
	mark=otimes,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_11.csv};

	\addplot[ % RoomsSmall
	scatter,
	only marks,
	mark=x,
 mark size=\marksize,
 fill opacity=0.5,
	scatter/use mapped color={
    draw=black,
    fill=black,
	}
	]%
	table [col sep=comma,x=#2,y=#4] {#1_12.csv};



	\addplot[no marks] coordinates {(0.01,0.01) (2700,2700) };
	\addplot[no marks, densely dotted] coordinates {(0.01,0.1) (90,900)};
	\addplot[no marks, densely dotted] coordinates {(0.1,0.01) (900,90)};
	\end{axis}
	\end{tikzpicture}
}

